Synthesizing Conjunctive Queries for Code Search

This paper presents Squid, a new conjunctive query synthesis algorithm for searching code with target patterns. Given positive and negative examples along with a natural language description, Squid analyzes the relations derived from the examples by a Datalog-based program analyzer and synthesizes a conjunctive query expressing the search intent. The synthesized query can be further used to search for desired grammatical constructs in the editor. To achieve high efficiency, we prune the huge search space by removing unnecessary relations and enumerating query candidates via refinement. We also introduce two quantitative metrics for query prioritization to select the queries from multiple candidates, yielding desired queries for code search. We have evaluated Squid on over thirty code search tasks. It is shown that Squid successfully synthesizes the conjunctive queries for all the tasks, taking only 2.56 seconds on average.

==> abstract.tex <==
\section*{Abstract}
Container selection is one of the most critical aspects of developing high performance applications.
By understanding container interfaces and their interactions with application code, tools can find alternative containers which can achieve the same functionality in the application context.
Such a process demands the precise recognition of how the containers are actually being used.
Consequently, developers can replace container type by a light-weighted one without changing program functionality.

This paper presents the design and evaluation of FastAtlas, a static recommendation system that automatically recommends the efficient containers for a given program.
The traces of container interfaces are extracted statically to identify how the containers are used in the applications.
Combined with interface specification, the generated traces enable equational reasoning of container types, and then symbolic performance analysis for the traces.
More efficient container types are finally recommended to the programmers, based on which the applications can be transformed to more efficient ones with reduced execution time.
The empirical evaluation shows that FastAtlas is highly effective and achieves an average performance improvement of x\% and xx\% on real-world projects.

==> evaltime.tex <==

\begin{table}[]
	\centering
	%\vspace{3mm}
	\caption{The statistics of synthesizing queries}
	%\vspace{-3mm}
	\resizebox{0.85\linewidth}{!} 
	{
		\begin{tabular}{c|ccc|c|cc|cc|cc}
			\toprule[0.45mm]
				\multicolumn{1}{c|}{\multirow{2}{*}{ID}}     &     \multicolumn{1}{c}{\multirow{2}{*}{  \begin{tabular}[c]{@{}c@{}}Size of\\ $G_Q$      \end{tabular}}}&  \multicolumn{1}{c}{\multirow{2}{*}{\#$R_Q$}}  &  \multicolumn{1}{c|}{\multirow{2}{*}{$k$}}  &   \multicolumn{1}{c|}{\multirow{2}{*}{  \begin{tabular}[c]{@{}c@{}}Size of\\ $G_{\Gamma}[\mathcal{R}']$      \end{tabular}}}   &          \multicolumn{2}{c|}{\ToolName}& \multicolumn{2}{c|}{\ToolNameNRR} & \multicolumn{2}{c}{\ToolNameNQR} \\ \cline{6-11} 
			\multicolumn{1}{c|}{}  & 	\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &  \multicolumn{1}{c|}{}  &\multicolumn{1}{c|}{}  & Time(s) & Mem(MB)  & Time(s) & Mem(MB)  & Time(s) & Mem(MB) \\ \midrule
			1                    & (2, 1, 1)     &       1    &       1   & (10, 19)                  & 2.36       &   26.85       & 7.58    &        36.62      & 2.98 & 27.55\\
			2                    & (3, 2, 2)   &      1     &       1     & (9, 17)             & 2.37      &   27.00        & 7.87    &      36.76        & 3.14& 37.21\\
			3                    & (2, 1, 1)   &        1    &       1   & (10, 21)            & 2.30         &    26.88    & 8.32    &      37.29        & 2.74&28.19 \\
			4                    & (2, 2, 2)   &       1    &       1      & (10, 23)               & 2.50     &    26.98        & 7.98  &        36.96        & OOT& NA\\
			5                    & (3, 2, 2)  &      1      &       1      & (9, 29)                & 2.60    &    28.23         & 6.90  &     36.13           & OOT& NA\\
			$6$                 & (3, 2, 2)   &      1    &       2       & (9, 23)             & 2.31      &     27.19         & 7.59   &        36.64       & 15.22& 124.54\\
			$7$                    & (3, 2, 1)  &        1    &       2    & (9, 29)           & 2.76      &    27.05       & 8.11      &     36.36       & OOT& NA\\
			8                    & (2, 1, 1)  &      1    &       1       & (8, 29)            & 2.36   &    26.88          & 7.41   &      36.04         & 49.43&291.29\\
			9                    & (2, 1, 1)  &      1    &       1       & (10, 25)          & 2.20    &             26.80& 7.65     &       36.92      & 2.37& 27.54\\
			10                   & (2, 1, 2)  &      2      &       1     & (9, 29)            & 2.31     &     26.84        & 7.64   &        36.02       & 15.62&107.81 \\
			11                   & (1, 0, 2)  &      1     &       1       & (9, 23)          & 2.17   &    26.78           & 8.08    &      36.80        & 2.74& 27.70\\
			12                   & (1, 0, 1)  &        1    &       1     & (9, 22)          & 2.22    &    26.88          & 8.38  &      36.63          & 2.34& 28.17\\
			13                   & (1, 0, 1)  &        1     &       1     & (10, 21)       & 2.18      &            26.89& 8.11     &       36.19      & 2.78& 28.21\\
			14                   & (2, 1, 0)   &     2     &       1      & (9, 17)        & 2.24     &             26.94 & 7.67   &        36.54       & 2.75& 27.50\\
			15                   & (2, 1, 0)   &        2    &       1    & (10, 25)           & 2.31   &    27.11           & 7.05    &        35.70      & 2.87& 27.57\\
			16                   & (3, 2, 2)    &      1      &       1    & (11, 26)          & 2.36 &   27.50              & 8.21   &       37.04        & OOT& NA\\
			17                   & (3, 2, 1)     &       1   &       1     & (9, 20)         & 2.45    &    27.25          & 9.04     &      37.52       & OOT& NA\\
			18                   & (4, 3, 0)  &        1     &       1    & (11, 26)        & 3.23    &    27.65          & 11.44     &      38.25      & OOT&NA \\
			19                   & (3, 2, 1)    &      1     &       1     & (12, 30)             & 2.38    &    27.30          & 8.92   &      36.81         & OOT& NA\\
			$20$                   & (2, 2, 0)  &         1     &       2   & (11, 27)            & 2.42   &     27.31          & 7.92  &        36.73        & OOT& NA\\
			21                   & (2, 1, 2)   &          2  &       1    & (11, 28)            & 2.53  &       27.14         & 8.13     &      36.85       & OOT&NA \\
			22                   & (3, 2, 1)   &          1   &       1    & (12, 35)           & 2.42    &     27.23         & 8.67    &      36.97        & OOT& NA\\
			$23$                   & (2, 1, 0)  &          1   &       2    & (13, 33)        & 2.21    &     27.25         & 8.32   &       37.27        & 3.97&28.20 \\
			24                   & (2, 1, 2)   &       1    &       1     & (13, 35)            & 2.58    &     26.89         & 8.21   &       36.84        & OOT& NA\\
			25                   & (3, 2, 1)  &       2     &       1     & (11, 28)             & 2.46     &     27.02        & 8.12    &      36.80        & OOT&NA \\ \midrule
			Avg  &  &      &       &          & 2.41     &     27.11        & 8.13    &      36.75       & 8.38 & 62.42\\
			\bottomrule[0.45mm]
		\end{tabular}
	}
	\label{table:time}
	%\vspace{-4.5mm}
\end{table}



\begin{table}[]
	\centering
	%\vspace{3mm}
	\caption{The statistics of synthesizing queries}
	%\vspace{-3mm}
	\resizebox{0.85\linewidth}{!} 
	{
		\begin{tabular}{c|ccc|c|cc|cc|cc}
			\toprule[0.45mm]
			\multicolumn{1}{c|}{\multirow{2}{*}{ID}}     &     \multicolumn{1}{c}{\multirow{2}{*}{  \begin{tabular}[c]{@{}c@{}}Size of\\ $G_Q$      \end{tabular}}}&  \multicolumn{1}{c}{\multirow{2}{*}{\#$R_Q$}}  &  \multicolumn{1}{c|}{\multirow{2}{*}{$k$}}  &   \multicolumn{1}{c|}{\multirow{2}{*}{  \begin{tabular}[c]{@{}c@{}}Size of\\ $G_{\Gamma}[\mathcal{R}']$      \end{tabular}}}   &          \multicolumn{2}{c|}{\ToolName}& \multicolumn{2}{c|}{\ToolNameNRR} & \multicolumn{2}{c}{\ToolNameNQR} \\ \cline{6-11} 
			\multicolumn{1}{c|}{}  & 	\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &  \multicolumn{1}{c|}{}  &\multicolumn{1}{c|}{}  & Time(s) & Mem(MB)  & Time(s) & Mem(MB)  & Time(s) & Mem(MB) \\ \midrule
			1                    & (2, 1, 1)     &          1   & (10, 19)                  & 2.36             & 7.58   2      & 2.98 \\
			2                    & (3, 2, 2)   &        1     & (9, 17)             & 2.37        & 7.87    6        & 3.14\\
			3                    & (2, 1, 1)   &          1   & (10, 21)            & 2.30         & 8.32        & 2.74 \\
			4                    & (2, 2, 2)   &          1      & (10, 23)               & 2.50       & 7.98   & OOT\\
			5                    & (3, 2, 2)  &          1      & (9, 29)                & 2.60      & 6.90      & OOT\\
			$6$                 & (3, 2, 2)   &         2       & (9, 23)             & 2.31      & 7.59   & 15.22\\
			$7$                    & (3, 2, 1)  &            2    & (9, 29)           & 2.76  & 8.11     & OOT\\
			8                    & (2, 1, 1)  &       1       & (8, 29)            & 2.36      & 7.41  & 49.43\\
			9                    & (2, 1, 1)  &         1       & (10, 25)          & 2.20  & 7.65    & 2.37\\
			10                   & (2, 1, 2)  &           1     & (9, 29)            & 2.31         & 7.64 & 15.62 \\
			11                   & (1, 0, 2)  &          1       & (9, 23)          & 2.17       & 8.08     & 2.74\\
			12                   & (1, 0, 1)  &        1     & (9, 22)          & 2.22     & 8.38   & 2.34\\
			13                   & (1, 0, 1)  &          1     & (10, 21)       & 2.18     & 8.11    & 2.78\\
			14                   & (2, 1, 0)   &         1      & (9, 17)        & 2.24   & 7.67   & 2.75\\
			15                   & (2, 1, 0)   &          1    & (10, 25)           & 2.31    & 7.05   & 2.87\\
			16                   & (3, 2, 2)    &           1    & (11, 26)          & 2.36   & 8.21      & OOT\\
			17                   & (3, 2, 1)     &        1     & (9, 20)         & 2.45     & 9.04   & OOT\\
			18                   & (4, 3, 0)  &        1     &       1    & (11, 26)        & 3.23  & 11.44   & OOT\\
			19                   & (3, 2, 1)    &      1     & (12, 30)             & 2.38   & 8.92  & OOT\\
			$20$                   & (2, 2, 0)  &           2   & (11, 27)            & 2.42   & 7.92 & OOT\\
			21                   & (2, 1, 2)   &          1    & (11, 28)            & 2.53  & 8.13   & OOT \\
			22                   & (3, 2, 1)   &         1    & (12, 35)           & 2.42   & 8.67    & OOT\\
			$23$                   & (2, 1, 0)  &       2    & (13, 33)        & 2.21    & 8.32  & 3.97 \\
			24                   & (2, 1, 2)   &         1     & (13, 35)            & 2.58   & 8.21   & OOT\\
			25                   & (3, 2, 1)  &       1     & (11, 28)             & 2.46    & 8.12    & OOT\\ \midrule
			Avg  &  &      &       &          & 2.41     & 8.13   & 8.38 \\
			\bottomrule[0.45mm]
		\end{tabular}
	}
	\label{table:time}
	%\vspace{-4.5mm}
\end{table}





==> problem_formalization.tex <==
\section{Problem Formulation}
Container type recommendation refers to a broad class of problems with different optimization targets, including minimizing the consumption of time, memory and energy.
The goal of our work is to reduce the execution time, while the formulation of other instances are similar, and our approach can also be easily extended to these instances.

\subsection{Semantic Model of Container}
When using containers, we concern three types of properties.
The first one is the index-value correlation or key-value correlation, which reflects the inner storage of position dependent containers, such as List, or value dependent containers, such as set and map.
The second one is the ownership of an elements, and we often care whether an element has been added in the container or not.
The third one is the size of the container, and the empty check or size comparison commonly occurs in the branch condition.
If the interfaces have the same effect on these three properties, we can regards them as the equivalent interfaces.
This inspires us to define semantic set and interface embedding for a container type $T$ as follows.

\begin{defn}
	A \emph{semantic set} of $T$ is the set of semantic operations that $T$ supports.
\end{defn}
\begin{defn}
	An \emph{interface embedding} of container type $T$ is a mapping $e_T : I_T \rightarrow \mathbb{P}(S_T)$ where $S_T$ is the semantic set of $T$, and $I_T$ is the set of interfaces of $T$.
\end{defn}

\begin{newexample}
	For java.util.Vector, the semantic set is 
	$$S_{vector} = \{ \varheart_b, \varheart_e, \varheart_r, \vardiamond_b, \vardiamond_e, \vardiamond_r, \varsuit_b,  \varsuit_e,  \varsuit_r, $$
	$$\vartriangle, \triangledown, \ominus, contains, size\}$$
	$\varheart$, $\vardiamond$ and $\varsuit$ represent the insertion, access and removal of a vector, and each kind of operations can occurs at the beginning, end or a random location of the vector.
	The size of a vector can be increased by one, decreased by one or unchanged under some operations, denoted by $\vartriangle$, $\triangledown$ and $\ominus$ respectively.
	Besides, java.util.Vector also supports ownership checking and inspection of the size.
	
	\noindent With this semantic set defined, we can naturally define the interface embedding $e_{vector}$.
	Obviously, it maps the interface $push\_back$ to 
	$$e_{vector}(push\_back) = \{\varheart_e, \vartriangle\}$$
\end{newexample}

Semantic set and interface embedding actually induce an abstraction of container interfaces.
The functionality of a container is determined by its semantic set, which means that if an interface of container type $T_1$ and another interface of $T_2$ are embedded to the same set, they have the same behavior and are exchangeable.
One typical example is \emph{push\_back} of \emph{Vector} and \emph{add} of \emph{Stack} in Java Collection Framework.

\yao{how are the symbols used below}

\subsection{Metamorphic Container}
\yao{what does metaxx conainer mean (informally), and what does they mean}
Based on the semantic set $S_T$ and the interface set $I_T$, we can define the traces of interfaces and metamorphic traces formally as follows.
\begin{defn}
	Given a container type $T$, a \emph{trace} of a container object with the type $T$ is a sequence of container interfaces, i.e., $tr = (i_1, i_2, \cdots, i_{l})$ where $\forall 1 \leq k \leq l$, $i_k \in I_T$. 
	$I_T$ is the set consisting of all interfaces of $T$.
\end{defn}
\begin{defn}
	Given two traces $tr_1 = (i_1^1, i_2^1, \cdots , i_{l}^1)$ and $tr_2 = (i_1^2, i_2^2, \cdots , i_{l}^2)$ of $T_1$ and $T_2$ respectively, $tr_1$ and $tr_2$ are \emph{metamorphic traces} iff they belong to one of the following three types
	\begin{itemize}[leftmargin=*]
		\item Type 1: Interfaces are semantically equivalent, i.e., 
		$$\forall 0 \leq k \leq l, \; e_{T_1}(i_k^1) = e_{T_2}(i_k^2)$$
		\item Type 2: Interfaces are equivalent w.r.t ownership, i.e., for all k, $i_k^1$ inserts an element iff $i_k^2$ also inserts an element.
		Additionally, we restrict that no interface accesses and removes the elements in containers.
		\item Type 3: Interfaces are equivalent w.r.t. size, i.e., for all k, $i_k^1$ changes the size of container by $\delta$ iff $i_k^2$ increases the size of container by $\delta$, where $\delta = \pm 1, 0$.
		Additionally, we restrict that no interface accesses the elements in containers.
	\end{itemize}
\end{defn}

The definition of metamorphic traces are consistent with our common usage of containers.
Index/Key-value correlation, ownership and size partition the traces into several sets of traces, and the traces in each set are metamorphic, which means that they can yield the same property.
Hence, the exchanging of container types which have metamorphic traces does not change the functionality of the program.
We have the following theorem formally.

\begin{newtheorem}
	Given a program P and a container object $o$ in P, the container type of $o$, named $T_1$, can be replaced by $T_2$ iff for each trace of $o$ in $P$, the interfaces of  $T_2$ can form a corresponding metamorphic trace.
	We call $T_2$ the metamorphic container type of $T_1$.
\end{newtheorem}

\subsection{A Satisfiability Problem on Metamorphic Containers}
Finally, the container recommendation problem can be formulated as the following satisfiability problem.
\begin{problem}
	Assume we have a set of container types $\mathcal{T}= \{T_1, T_2, ..., T_n\}$ and an application $P$ to be optimized. 
	For each container type, we have its semantic set $S_{T_i}$ and its interface embedding $e_{T_i}$.
	The partial order $\preceq \subseteq I \times I$ defines the complexity order of interfaces, where $I = \bigcup_{1 \leq k \leq n} I_{T_k}$.
	For a container object $o$ with type $T_j \in A$, finding a more efficient container type is equivalent to answer whether there exists another container type $T_k \in A$, such that
	\begin{itemize}[leftmargin=*]
		\item \textbf{Semantics condition.}
		$T_k$ can form a trace metamorphic to any given trace of $o$ in the application $P$.
		\item \textbf{Performance condition.}
		For any pair of metamorphic traces $tr_1 = (i_1^1, i_2^1, \cdots , i_{l}^1)$ and $tr_2 = (i_1^2, i_2^2, \cdots , i_{l}^2)$, where $i_s^1 \in I_{T_j}$ and $i_s^2 \in I_{T_k}$, $i_s^2 \preceq i_s^1$ always holds for all $1 \leq s \leq l$ and there exists $1 \leq s_0 \leq l$ such that $i_s^1 \npreceq i_s^2$
	\end{itemize}
\end{problem}
Specifically, semantic condition guarantees the functional correctness, i.e.,  the functionality of program must be preserved if programmers replace original container type by the recommended one.
Performance condition assures the recommended container type behave better than the original one in terms of efficiency.

\yao{what are the challenges/difficulities}
\yao{what are your program abstractions}

==> refineRule.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.45\linewidth}
\centering
\[
\footnotesize
\inference
{
N_Q = \{(R^{*}, A_1)\}, G_Q = (N_Q, \emptyset, \bot)
}
{
\mathcal{R}', (N_{\Gamma}, E_{\Gamma}), (R_p^{*}, R_n^{*}) \vdash \kappa^{-1}(G_Q ) \in \mathcal{S}_R(1, 1)
}
\]
\quad \footnotesize(\textsc{Base})
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.53\linewidth}
\centering
\[
\footnotesize
\inference
{
R_Q \in \mathcal{S}_R(m, k), \ \Pi_{(R_p^{*}.*)}(R_p^{*}) = \Pi_{(A_1.*)}(R_Q)   \\
}
{
\mathcal{R}', (N_{\Gamma}, E_{\Gamma}), (R_p^{*}, R_n^{*}) \vdash R_Q \in \mathcal{S}_C(m, k)
}
\]
\quad \footnotesize (\textsc{CheckCandidate})
\end{subfigure}

%\vspace{2.5mm}



\begin{subfigure}[b]{0.5\linewidth}
	\centering
	\[
	\footnotesize
	\inference
	{
		R_Q \in \mathcal{S}_R(m-1, k-1),  \ (N_Q, \ E_Q, \ \Phi_Q) = \kappa(R_Q)\\
		R \in \mathcal{R}', \ | \{(R, A_i)\in N_Q  \}| = k-1\\
		G_Q' = (N_Q \cup \{(R, A_{|N_Q|+1}) \}, E_Q, \ \Phi_Q)\\
	}
	{
		\mathcal{R}', (N_{\Gamma}, E_{\Gamma}), (R_p^{*}, R_n^{*}) \vdash \kappa^{-1}(G_Q') \in \mathcal{S}_R(m, k)
	}
	\]
	\quad \footnotesize(\textsc{AddRelation-I})
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.46\linewidth}
	\centering
	\[
	\footnotesize
	\inference
	{
		R_Q \in \mathcal{S}_R(m-1, k),  \ (N_Q, \ E_Q, \ \Phi_Q) = \kappa(R_Q)\\
		R \in \mathcal{R}', \ | \{(R, A_i)\in N_Q  \}| < k\\
		G_Q' = (N_Q \cup \{(R, A_{|N_Q|+1}) \}, E_Q, \ \Phi_Q)\\
	}
	{
		\mathcal{R}', (N_{\Gamma}, E_{\Gamma}), (R_p^{*}, R_n^{*}) \vdash \kappa^{-1}(G_Q') \in \mathcal{S}_R(m, k)
	}
	\]
	\quad \footnotesize(\textsc{AddRelation-II})
\end{subfigure}

%\vspace{2.5mm}
\centering
\begin{subfigure}[b]{0.75\linewidth}
\centering
\[
\footnotesize
\inference
{
R_Q \in \mathcal{S}_R(m, k),  \ (N_Q, \ E_Q, \ \Phi_Q) = \kappa(R_Q), \ (R_i, R_j, a) \in E_{\Gamma}\\
n_i = (R_i, A_i) \in N_Q, \ n_j = (R_j, A_j) \in N_Q, \ e=(n_i, n_j, a) \notin E_Q\\
G_Q' = (N_Q, E_Q \cup \{e\}, \Phi_Q), \ R_Q' = \kappa^{-1}(G_Q'), \ \ \Pi_{(R_p^{*}.*)}(R_p^{*}) \subseteq \Pi_{(A_1.*)}(R_Q')
}
{
\mathcal{R}', (N_{\Gamma}, E_{\Gamma}), (R_p^{*}, R_n^{*}) \vdash R_Q' \in \mathcal{S}_R(m, k)
}
\]
\quad \footnotesize(\textsc{AddEqCon})
\end{subfigure}

\begin{subfigure}[b]{0.9\linewidth}
\centering
\[
\footnotesize
\inference
{
R_Q \in \mathcal{S}_R(m, k),  \ (N_Q, \ E_Q, \ \Phi_Q) = \kappa(R_Q), \ (R, A) \in N_Q, \ (R, \textsf{STR}, a) \in E_{\Gamma} \\
%(R, A, a) \notin dom(\Phi_Q) \\
\Phi_Q' = \Phi_Q [(R, A, a) \mapsto \textsc{SynSCon}(R_Q, R, A, a)], \ G_Q' = (N_Q, E_Q, \Phi_Q'), \ R_Q' = \kappa^{-1}(G_Q')
}
{
\mathcal{R}', (N_{\Gamma}, E_{\Gamma}), (R_p^{*}, R_n^{*}) \vdash R_Q' \in \mathcal{S}_R(m, k)
}
\]
	\quad \footnotesize(\textsc{AddStrCon})
\end{subfigure}

%\vspace{2.5mm}

\begin{subfigure}[b]{0.95\linewidth}
\centering
\[
\footnotesize
\inference
{
R_Q' = R_Q[R_p^{*} / R^{*}], \ S_{\textsf{str}} = \Pi_{(A.a)}(R_Q'), \ (p, \ell) = \textsf{LCS}(S_{\textsf{str}}), \ p \in \{\textsf{equal}, \textsf{suffix}, \textsf{prefix}, \textsf{contain}\}
}
{
\mathcal{R}', (N_{\Gamma}, E_{\Gamma}), (R_p^{*}, R_n^{*}) \vdash \textsc{SynSCon}(R_Q, R, A, a): (p, \ell)
}
\]
\quad \footnotesize(\textsc{SynSCon})

\end{subfigure}
%\vspace{-6mm} 
\caption{Rules of the query refinement }
\vspace{-3mm} 
\label{fig:rule}
\end{figure*}

==> related_work.tex <==
\section{Related Work}

\textbf{Container selection.}
There have been a body of work attempting to detect and optimize inefficient container usage.
ARTEMIS~\cite{basios2018darwinian} and SEEDS~\cite{manotas2014seeds} convert the selection of optimal container type to an optimization problem.
Both of them defines the searching space by generalizing the original container type specified by developers according to the class hierarchy diagram.
For example, \emph{Stack}  is the subclass of \emph{Vector} in Java Collection Framework, and they state it is feasible to replace \emph{Stack} by \emph{Vector} if only the methods in \emph{Vector} are used.
This observation induces the searching space, in which the optimal container type can be found out by replacing original type exhaustively followed by dynamic profiling.
Different from them, our approach does not rely on class hierarchy diagram and is able to discover the candidates in various types, such as numeric types.

\textbf{Performance analysis.}
Contrast to program correctness bugs, performance bugs are often too vague to establish a methodology to detect them because of the lack of oracle.
Dynamic approaches are effective to exercise program to reach the peak resource consumption~\cite{slowFuzz}, but cannot provide the evidence that a performance bug exists or an alternative implementation with better performance.
Static approaches can detect the inefficient patterns based on manual observation~\cite{Dillig15ContainerTraversal, Song17PerformanceLoop}, while the preknowledge is often uneasy to be obtained.
In our work, we aims to the problem of container type selection, which is a subproblem of performance analysis.
An non-trivial quotient trace space indicates the possibility of optimization, which can be taken as the oracle of this subproblem in the big picture of performance analysis.

\textbf{Data structure specification.}
Data structure specification generation and verification are the fundamental problems in program language research.
Logic methods based shape analysis shed the sight of verify the functional correctness of data structure interfaces~\cite{Thomas02Parametric, Yang11BiAbduction}.
Recently, Grasshopper verifies the property of a data structure interface by inspecting separation logic formulae~\cite{Wies13Logic, Wies18Compositional}.
Multiple-domain properties, including size and element order, can also be checked by more powerful automatic reasoning system~\cite{Rinard08FullSpec, Rinard09Language, Gulwani09PartitionSize}.
Our work shows the possibility of utilizing verification as pre-analysis to guide the code transformation for certain purposes, such as performance optimization.

\textbf{Code transformation.}
Code transformation is a common interest in multiple fields of programming languages and software engineering, including compiler optimization, code search, code refactoring, etc.
Compilers can transform particular program structures to equivalent code snippet with lower complexity.
For example, Clang can transform the collective and inductive integer loop to its closed form.
%cite, %Numeric loop summarization
More sophisticated transformation involves data structures, such as array, stream and string.
For example, SIGMA summarizes collective operations in loops to support program verification, equivalence checking and translating program to high-performance~\cite{Guannan19CollectiveOp}.
Moller presents an ahead-of-time bytecode-to-bytecode transformation to optimize Java Stream Pipeline, which is promising to eliminate abstraction overhead~\cite{Moller20StreamPipepline}.
Besides, string loops with some properties can be replaced by string APIs, of which the semantics can be encoded by constraint in string theory.
Such transformation makes it possible to apply other program analysis techniques, such as symbolic execution, to analyze some particular forms of string loops precisely, and take advantages of string API optimization in compilers~\cite{Cadar19StringRefactoring}.
Similarly, we also face the necessity of assuring the equivalence of program in container type replacement.
However, type replacement means that whole program analysis is unavoidable to draw the boundary of optimization, while existing works on code transformation mainly focus on the local program patterns, such as particular types of loops and statements, and miss the chance of global optimization.
%Semantic code search, PLDI 2020


